Quantum Unpredictability

Unpredictable functions (UPFs) play essential roles in classical cryptography, including message authentication codes (MACs) and digital signatures. In this paper, we introduce a quantum analog of UPFs, which we call unpredictable state generators (UPSGs). UPSGs are implied by pseudorandom function-like states generators (PRFSs), which are a quantum analog of pseudorandom functions (PRFs), and therefore UPSGs could exist even if one-way functions do not exist, similar to other recently introduced primitives like pseudorandom state generators (PRSGs), one-way state generators (OWSGs), and EFIs. In classical cryptography, UPFs are equivalent to PRFs, but in the quantum case, the equivalence is not clear, and UPSGs could be weaker than PRFSs. Despite this, we demonstrate that all known applications of PRFSs are also achievable with UPSGs. They include IND-CPA-secure secret-key encryption and EUF-CMA-secure MACs with unclonable tags. Our findings suggest that, for many applications, quantum unpredictability, rather than quantum pseudorandomness, is sufficient.

==> reusable.tex <==
% !TEX root = main.tex
\section{Recyclable Variant}\label{sec:recyclable}
In the construction given in \cref{sec:construction}, a quantum public key can be used to encrypt only one message and a sender needs to obtain a new quantum public key whenever it encrypts a message. This is not desirable from practical perspective. 
In this section, we define recyclable QPKE where a sender only needs to receive one quantum public key to send arbitrarily many messages. The definition is similar to QPKE as defined in~\cref{def:QPKE} except that the encryption algorithm outputs a classical \emph{recycled} key that can be reused to encrypt messages many times.   
%In this section, we show that we can upgrade the scheme into a reusable one where a single quantum public key can be used to encrypt arbitrarily many messages. 

%We define reusable QPKE. The definition is similar to \cite{cryptoeprint:2023/345} with a crucial difference that we allow adversaries to tamper with quantum public keys.

%\takashi{I revised the definition to deal with the issue that an adversary may send a recycled key to the sender.}
\begin{definition}[Recyclable QPKE]
A recyclable QPKE scheme with message space $\bit^\ell$ is a set of algorithms  $(\SKGen,\PKGen,\Enc,\rEnc,\Dec)$ such that
\begin{itemize}
    \item 
    $\SKGen(1^\secp)\to (\sk,\vk):$
    It is a PPT algorithm that, on input the security parameter $\secp$, outputs
    a classical secret key $\sk$ and a classical verification key $\vk$. 
    \item
    $\PKGen(\sk)\to \pk:$
    It is a QPT algorithm that, on input $\sk$, outputs
    a quantum public key $\pk$.
    \item
    $\Enc(\vk,\pk,\msg)\to (\ct,\rk):$ 
    It is a QPT algorithm that, on input $\vk$, $\pk$, and a plaintext $\msg\in\bit^\ell$, outputs a classical ciphertext $\ct$ and classical recycled key $\rk$.  
    \item
    $\rEnc(\rk,\msg)\to \ct:$ 
    It is a PPT algorithm that, on input $\rk$ and a plaintext $\msg\in\bit^\ell$, outputs a classical ciphertext $\ct$. 
    \item
    $\Dec(\sk,\ct)\to \msg':$ 
    It is a classical deterministic polynomial-time algorithm that, on input $\sk$ and $\ct$, outputs $\msg'\in\bit^\ell \cup \{\bot\}$.
\end{itemize}


We require the following correctness and IND-pkTA security.

\paragraph{\bf Correctness:}
 For any $\msg,\msg'\in\bit^\ell$,
\begin{equation}
   \Pr\left[
   \msg\gets\Dec(\sk,\ct)
   \land\\ 
   \msg'\gets\Dec(\sk,\ct'):
   \begin{array}{r}
   (\sk,\vk)\gets\SKGen(1^\secp)\\
   \pk\gets\PKGen(\sk)\\
   (\ct,\rk)\gets\Enc(\vk,\pk,\msg)\\
   \ct'\gets\rEnc(\rk,\msg')
   \end{array}
   \right] \ge 1-\negl(\secp).
\end{equation}

\paragraph{\bf IND-pkTA security under quantum public keys:}
For any polynomial $m$, and any QPT adversary $\cA$,
\begin{equation}
   \Pr\left[b\gets\cA^{\rEnc(\rk,\cdot)}(\ct^\ast ,\st):
   \begin{array}{r}
   (\sk,\vk)\gets\SKGen(1^\secp)\\
   \pk_1,...,\pk_m\gets\PKGen(\sk)^{\otimes m}\\
   (\pk',\msg_0,\msg_1,\st)\gets\cA(\vk,\pk_1,...,\pk_m)\\
   b\gets \bit\\ 
   (\ct^\ast,\rk) \gets\Enc(\vk,\pk',\msg_b)
   \end{array}
   \right] \le \frac{1}{2}+\negl(\secp).
\end{equation}
Here, $\pk_1,...,\pk_m\gets\PKGen(\sk)^{\otimes m}$
means that $\PKGen$ is executed $m$ times and $\pk_i$ is the output of the $i$th execution of $\PKGen$, $\rEnc(\rk,\cdot)$ means a classically-accessible encryption oracle,
and $\st$ is a quantum internal state of $\cA$, which can be entangled with $\pk'$.


\paragraph{\bf IND-pkTA security under recycled keys:} 
For any polynomial $m$, and any QPT adversary $\cA$,
\begin{equation}
   \Pr\left[b\gets\cA^{\rEnc(\rk,\cdot)}(\ct^\ast ,\st'):
   \begin{array}{r}
   (\sk,\vk)\gets\SKGen(1^\secp)\\
   \pk_1,...,\pk_m\gets\PKGen(\sk)^{\otimes m}\\
   (\pk',\msg,\st)\gets\cA(\vk,\pk_1,...,\pk_m)\\
   (\ct,\rk) \gets\Enc(\vk,\pk',\msg)\\
    (\msg_0,\msg_1,\st')\gets \cA^{\rEnc(\rk,\cdot)}(\ct,\st)\\ 
   b\gets \bit\\ 
   \ct^\ast \gets\rEnc(\rk,\msg_b)
   \end{array}
   \right] \le \frac{1}{2}+\negl(\secp).
\end{equation}
Here, $\pk_1,...,\pk_m\gets\PKGen(\sk)^{\otimes m}$
means that $\PKGen$ is executed $m$ times and $\pk_i$ is the output of the $i$th execution of $\PKGen$,  $\rEnc(\rk,\cdot)$ means a classically-accessible encryption oracle, 
and $\st$ and $\st'$ are quantum internal states of $\cA$, which can be entangled with $\pk'$.
%that returns $\rEnc(\rk,\msg)$ on input $\msg$. 
\end{definition}




\iffalse
\begin{definition}[Reusable QPKE]
A reusable QPKE scheme $(\SKGen,\PKGen,\Enc,\Dec)$ with message space $\bit^\ell$ has similar syntax to QPKE as defined in \cref{def:QPKE} except that the encryption algorithm additionally outputs a (possibly quantum) recycled public key in addition to a ciphertext.\footnote{In our construction, recycled public keys are classical.}    
We write $(\ct,\tilde{\pk})\gets \Enc(\msg,\vk,\pk)$ to mean that the encryption algorithm outputs a ciphertext $\ct$ and a recycled key $\tilde{\pk}$. 
We require the following reusable correctness and reusable IND-CPA security.

\paragraph{\bf Reusable correctness:}
For any polynonmial $k$ and $\msg^{(1)},...,\msg^{(k)}\in\bit^\ell$, 
\begin{equation}
   \Pr\left[\msg^{(k)}\gets\Dec(\ct^{(k)},\sk):
   \begin{array}{r}
   (\sk,\vk)\gets\SKGen(1^\secp)\\
   \pk^{(1)}\gets\PKGen(\sk)\\
   \textrm{For~}i=1,2,...,k, (\ct^{(i)},\pk^{(i+1)})\gets\Enc(\vk,\pk^{(i)},\msg^{(i)})\\
   \end{array}
   \right] \ge 1-\negl(\secp).
\end{equation}

\paragraph{\bf Reusable IND-CPA security:}
For any polynomials $m$ and $k$, and any QPT adversary $\cA$, consider the following experiment between $\cA$ and the challenger $\cC$:
\begin{enumerate}
    \item $\cC$ generates $(\sk,\vk)\gets\SKGen(1^\secp)$ and $\pk_1,...,\pk_m\gets\PKGen(\sk)^{\otimes m}$ where $\pk_1,...,\pk_m\gets\PKGen(\sk)^{\otimes m}$
means that $\PKGen$ is executed $m$ times and $\pk_i$ is the output of the $i$th execution of $\PKGen$, and sends $(\vk,\pk_1,...,\pk_m)$ to $\cA$.
\item $\cA$ sends a tampered public key $\pk'$ to $\cC$.
\item $\cC$ lets $\pk^{(1)}:=\pk'$. \takashi{Technically, I could simply say that "$\cA$ sends a tampered public key $\pk^{(1)}$ to $\cA$" in the previous bullet point. Is that better?}\mor{I prefer the current one.}
\item For $i=1,...,k-1$, do the following:
\begin{enumerate}
    \item $\cA$ sends a message $\msg^{(i)}$ to $\cC$.
    \item $\cC$ generates $(\ct^{(i)},\pk^{(i+1)})\gets\Enc(\vk,\pk^{(i)},\msg^{(i)})$ and sends $\ct^{(i)}$ to $\cA$. 
\end{enumerate}
\item $\cA$ sends a challenge message pair $(\msg^{(k)}_0,\msg^{(k)}_1)\in \bit^{\ell\times 2}$ to $\cC$.
\item $\cC$ picks $b\gets \bit$, generates $(\ct^{(k)},\pk^{(k+1)})\gets\Enc(\vk,\pk^{(k)},\msg^{(k)})$ and sends $\ct^{(k)}$ to $\cA$.
\item $\cA$ outputs a bit $b'$.
\end{enumerate}
In the above experiment, we have 
\begin{equation}
   \Pr[b'=b]\le \frac{1}{2}+\negl(\secp).
\end{equation}
\end{definition}
\fi

\paragraph{Construction.} 
We show a generic construction of recyclable QPKE from (non-recyclable) QPKE with classical ciphertexts and IND-CPA secure SKE via standard hybrid encryption.  

Let $\QPKE=(\QPKE.\SKGen,\QPKE.\PKGen,\QPKE.\Enc,\QPKE.\Dec)$ be a (non-recyclable) QPKE scheme with message space $\bit^\secp$ and $\SKE=(\SKE.\Enc,\SKE.\Dec)$ be an SKE scheme with message space $\bit^\ell$. Then we construct a recyclable QPKE scheme $\QPKE'=(\QPKE'.\SKGen,\QPKE'.\PKGen,\QPKE'.\Enc,\allowbreak \QPKE'.\rEnc,\QPKE'.\Dec)$ with message space $\bit^\ell$ as follows:
\begin{itemize}
    \item 
    $\QPKE'.\SKGen(1^\secp)\to (\sk',\vk'):$
    Run  $(\sk,\vk)\gets \QPKE.\SKGen(1^\secp)$ and output a secret key $\sk':=\sk$ and verification key $\vk':=\vk$. 
    \item
    $\QPKE'.\PKGen(\sk')\to \pk':$
    Run $\pk \gets \QPKE.\PKGen(\sk)$ and outputs $\pk':=\pk$. 
    \item
    $\QPKE'.\Enc(\vk',\pk',\msg)\to (\ct',\rk'):$
        Parse $\pk'=\pk$ and $\vk'=\vk$,  
        sample $K\gets \bit^\secp$,  run  $\ct \gets \QPKE.\Enc(\vk,\pk,K)$ and $\ct_{\ske}\gets \SKE.\Enc(K,\msg)$, and output a ciphertext $\ct':=(\ct,\ct_{\ske})$ and recycled key $\rk':=(K,\ct)$.
 \item
 $\QPKE'.\rEnc(\rk',\msg)\to \ct':$
Parse $\rk'=(K,\ct)$, run $\ct_{\ske}\gets \SKE.\Enc(K,\msg)$, and output a ciphertext $\ct':=(\ct,\ct_{\ske})$. 
    \item
    $\QPKE'.\Dec(\sk',\ct')\to \msg':$
    Parse $\ct'=(\ct,\ct_{\ske})$ and $\sk'=\sk$, run $K'\gets \QPKE.\Dec(\sk,\ct)$ and $\msg' \gets \SKE.\Dec(K',\ct_{\ske})$, and output $\msg'$. 
\end{itemize}

\paragraph{Correctness.}
Correctness of $\QPKE'$ immediately follows from correctness of $\QPKE$ and $\SKE$. 

\paragraph{IND-pkTA security.}
IND-pkTA security of $\QPKE$ implies that the SKE key $K$ chosen by $\QPKE'.\Enc$ is computationally indistinguishable from uniformly random for an adversary. Then IND-CPA security of $\SKE$ directly implies IND-pkTA security under quantum public keys and recycled keys of $\QPKE'$ 
since $\msg$ is encrypted by $\SKE$ under the key $K$ in both of  $\QPKE'.\Enc$ and $\QPKE'.\rEnc$. 
%When $k\geq 2$, the challenge message pair will be encrypted under a recycled public key $\tilde{\pk}=(1,K,\ct)$ where $K$ is computationally indistinguishable from uniformly random as

\begin{remark}
We can generically add decryption error detectability by using digital signatures similarly to (non-recyclable) QPKE. 
\end{remark}
